Entropy- and Distance-Based Predictors From GPT-2 Attention Patterns Predict Reading Times Over and Above GPT-2 Surprisal

Transformer-based large language models are trained to make predictions about the next word by aggregating representations of previous tokens through their self-attention mechanism. In the field of cognitive modeling, such attention patterns have recently been interpreted as embodying the process of cue-based retrieval, in which attention over multiple targets is taken to generate interference and latency during retrieval. Under this framework, this work first defines an entropy-based predictor that quantifies the diffuseness of self-attention, as well as distance-based predictors that capture the incremental change in attention patterns across timesteps. Moreover, following recent studies that question the informativeness of attention weights, we also experiment with alternative methods for incorporating vector norms into attention weights. Regression experiments using predictors calculated from the GPT-2 language model show that these predictors deliver a substantially better fit to held-out self-paced reading and eye-tracking data over a rigorous baseline including GPT-2 surprisal. Additionally, the distance-based predictors generally demonstrated higher predictive power, with effect sizes of up to 6.59 ms per standard deviation on self-paced reading times (compared to 2.82 ms for surprisal) and 1.05 ms per standard deviation on eye-gaze durations (compared to 3.81 ms for surprisal).

==> scratch.tex <==
% present average?
% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.073888 ($p<0.001$) & 0.073930 ($p<0.001$) & 0.073433 ($p<0.001$) & 0.073807 ($p<0.001$) \\
%     {\sc Attn-N} & 0.073600 ($p<0.001$) & 0.074111 ($p=0.055$) & 0.073500 ($p<0.001$) & 0.074086 ($p=0.016$) \\
%     {\sc AttnRL-N} & 0.073559 ($p<0.001$) & 0.074115 ($p=0.009$) & 0.073624 ($p<0.001$) & 0.072647 ($p<0.001$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the exploratory partition of the Natural Stories Corpus. No random effects baseline MSE: 0.074239}
%     \label{tab:exp1_noint_expl}
% \end{table*}

% present average?
% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.067559 ($p=0.012$) & 0.067613 ($p<0.001$) & 0.067678 ($p=0.291$) & 0.067820 ($p=1$) \\
%     {\sc Attn-N} & 0.067300 ($p<0.001$) & 0.067690 ($p=0.002$) & 0.067623 ($p=0.097$) & 0.067688 ($p=0.002$) \\
%     {\sc AttnRL-N} & 0.067346 ($p<0.001$) & 0.067653 ($p<0.001$) & 0.067355 ($p<0.001$) & 0.067234 ($p<0.001$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the exploratory partition of the Natural Stories Corpus. Random intercept only baseline MSE: 0.067801}
%     \label{tab:exp1_int_expl}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.073806 ($p<0.001$) & 0.073953 ($p<0.001$) & 0.073581 ($p<0.001$) & 0.073848 ($p<0.001$) \\
%     {\sc Attn-N} & 0.073472 ($p<0.001$) & 0.074065 ($p=0.009$) & 0.073646 ($p<0.001$) & 0.074073 ($p=0.0181$) \\
%     {\sc AttnRL-N} & 0.073441 ($p<0.001$) & 0.074150 ($p=0.1831$) & 0.073738 ($p<0.001$) & 0.072429 ($p<0.001$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the held-out partition of the Natural Stories Corpus. Baseline MSE: 0.074213}
%     \label{tab:exp1_held}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.229435 ($p=0.0344$) & 0.229003 ($p<0.001$) & 0.228890 ($p<0.001$) & 0.228911 ($p<0.001$) \\
%     {\sc Attn-N} & 0.229473 ($p=0.2829$) & 0.229080 ($p<0.001$) & 0.228759 ($p<0.001$) & 0.229037 ($p<0.001$) \\
%     {\sc AttnRL-N} & 0.229500 ($p=1$) & 0.229057 ($p<0.001$) & 0.228855 ($p<0.001$) & 0.229012 ($p<0.001$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the exploratory partition of the Dundee Corpus. No random effects baseline MSE: 0.229492}
%     \label{tab:exp2_noint_expl}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.223877 ($p<0.001$) & 0.223765 ($p=0.071$) & 0.223801 ($p=0.112$) & 0.223787 ($p=0.091$) \\
%     {\sc Attn-N} & 0.223910 ($p<0.001$) & 0.223347 ($p<0.001$) & 0.223595 ($p=0.007$) & 0.223343 ($p<0.001$) \\
%     {\sc AttnRL-N} & 0.223924 ($p=0.002$) & 0.223366 ($p<0.001$) & 0.223188 ($p<0.001$) & 0.224058 ($p=1$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the exploratory partition of the Dundee Corpus. Random intercept only baseline MSE: 0.224044}
%     \label{tab:exp2_int_expl}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     % \footnotesize
%     \begin{tabular}{r r r r r}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c}{Predictors} \\
%     \cmidrule{2-5}
%     & NAE & $\Delta$NAE & MD & EMD \\
%     \midrule
%     {\sc Attn-W} & 0.227143 ($p=0.023$) & 0.226479 ($p<0.001$) & 0.226407 ($p<0.001$) & 0.226443 ($p<0.001$) \\
%     {\sc Attn-N} & 0.227174 ($p=0.047$) & 0.226572 ($p<0.001$) & 0.226202 ($p<0.001$) & 0.226545 ($p<0.001$) \\
%     {\sc AttnRL-N} & 0.227235 ($p=1$) & 0.226531 ($p<0.001$) & 0.226333 ($p<0.001$) & 0.226952 ($p=0.004$) \\
%     \bottomrule
%     \end{tabular}
%     \caption{MSE on the held-out partition of the Dundee Corpus. Baseline MSE: 0.227210}
%     \label{tab:exp2_held}
% \end{table*}
